NetDiffusion: Network Data Augmentation Through Protocol-Constrained Traffic Generation

Datasets of labeled network traces are essential for a multitude of machine learning (ML) tasks in networking, yet their availability is hindered by privacy and maintenance concerns, such as data staleness. To overcome this limitation, synthetic network traces can often augment existing datasets. Unfortunately, current synthetic trace generation methods, which typically produce only aggregated flow statistics or a few selected packet attributes, do not always suffice, especially when model training relies on having features that are only available from packet traces. This shortfall manifests in both insufficient statistical resemblance to real traces and suboptimal performance on ML tasks when employed for data augmentation. In this paper, we apply diffusion models to generate high-resolution synthetic network traffic traces. We present NetDiffusion, a tool that uses a finely-tuned, controlled variant of a Stable Diffusion model to generate synthetic network traffic that is high fidelity and conforms to protocol specifications. Our evaluation demonstrates that packet captures generated from NetDiffusion can achieve higher statistical similarity to real data and improved ML model performance than current state-of-the-art approaches (e.g., GAN-based approaches). Furthermore, our synthetic traces are compatible with common network analysis tools and support a myriad of network tasks, suggesting that NetDiffusion can serve a broader spectrum of network analysis and testing tasks, extending beyond ML-centric applications.

==> future.tex <==
\section{Future Work}\label{sec:future}
\paragraph{Embedding Protocol-Rule Constraints in Generation.}
Our current approach leans on post-generation heuristics to
achieve protocol rule-compliance challenges posed by the diffusion generation process.
This choice arises from the inherent complexities of enforcing
protocol rule-compliant controls during the diffusion
generation process, which demands the intricate management of
inter-dependent constraints.
While post-generation heuristics offers a naive solution,
direct integration of these constraints during generation would be ideal.
Future endeavors will explore embedding these protocol rules
directly within the generation pipeline, circumventing the
need for post-hoc adjustments.

\paragraph{Inter-Packet Time Dependency. need better title}
Presently, our method samples timestamps from original distributions
post-generation,
ensuring statistical resemblance to real data.
In the future, we aim to enhance diffusion models to learn time series directly,
providing a more generative approach for inter-packet time dependencies.

\paragraph{Scalability in Flow Size.}
The scope of our generation is currently limited to 1,024 packets
per sample, constrained by the capabilities of existing
text-to-image diffusion models, even with latent diffusion.
We aim to circumvent these limitations,
potentially by embracing tabular diffusion that retains packet
dependencies or through sequential flow generation.

\paragraph{Custom Foundation Model Training.}
Our methodology predominantly relies on fine-tuning pre-existing
base models. While this approach is effective,
there is potential in training a dedicated network-specific
diffusion foundation model from scratch,
enhancing generation accuracy.
However, such an endeavor would demand substantial
training data and computational resources.

\paragraph{Semantically-Meaningful Payload Generation.}
Generating payloads presents a unique challenge,
especially given that most are encrypted.
This encryption can complicate the diffusion model's learning
curve, making it difficult to produce semantically meaningful
payloads. Additionally, the sheer volume of data in payloads
poses representational challenges. A potential solution
could involve the use of autoencoders,
facilitating dimensionality reduction and the extraction of
critical payload attributes.
